Generalizing Face Forgery Detection with High-frequency Features

Current face forgery detection methods achieve high accuracy under the within-database scenario where training and testing forgeries are synthesized by the same algorithm. However, few of them gain satisfying performance under the cross-database scenario where training and testing forgeries are synthesized by different algorithms. In this paper, we find that current CNN-based detectors tend to overfit to method-specific color textures and thus fail to generalize. Observing that image noises remove color textures and expose discrepancies between authentic and tampered regions, we propose to utilize the high-frequency noises for face forgery detection. We carefully devise three functional modules to take full advantage of the high-frequency features. The first is the multi-scale high-frequency feature extraction module that extracts high-frequency noises at multiple scales and composes a novel modality. The second is the residual-guided spatial attention module that guides the low-level RGB feature extractor to concentrate more on forgery traces from a new perspective. The last is the cross-modality attention module that leverages the correlation between the two complementary modalities to promote feature learning for each other. Comprehensive evaluations on several benchmark databases corroborate the superior generalization performance of our proposed method.

==> figure/dataset.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=13cm]{figure/pdf/datasets.pdf} 
  \caption
    {Examples of real and fake images in each database.}
 \label{fig:dataset}
\end{figure}

==> figure/fig_spatial_dcma.tex <==
% \begin{figure}[t]
%   \centering
%     \begin{minipage}{.5\textwidth}
%         \centering
%         \includegraphics[width=1.0\linewidth]{figure/pdf/srm_sa.pdf} 
%         \caption{The residual guided spatial attention module.}
%         \label{fig:srm_sa}
%     \end{minipage}%
%     \hspace{1cm}
%     \begin{minipage}{0.4\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figure/pdf/dual_cma.pdf}
%  %   \vspace{-5pt}
%       \caption
%         {The dual cross-modality attention.}
%      \label{fig:dual_cma}
%     \end{minipage}
% \end{figure}


\begin{figure}[t]
    \centering
    \scalebox{0.85}{
    \includegraphics[width=\linewidth]{figure/pdf/srm_sa.pdf}}
    \caption{The residual guided spatial attention module.}
    \label{fig:srm_sa}
\end{figure}

\begin{figure}[t]
    \centering
    \scalebox{0.85}{
    \includegraphics[width=\linewidth]{figure/pdf/dual_cma.pdf}}
    \caption{The dual cross-modality attention.}
    \label{fig:dual_cma}
\end{figure}


==> figure/real-fake-example.tex <==
% TODO: 现在的阐释与我们的工作相关性不大，考虑做一个图显示不同造假的数据分布不同

\begin{figure}[!htp]
  \centering
  \includegraphics[width=0.65\linewidth]{figure/img/real-fake-example.png} 
  \caption
    {Face images from DeepFakeDetection dataset. The first column is pristine while the second column is manipulated.}
 \label{fig:real-fake-example}
\end{figure}

==> figure/varied-statistics.tex <==
\begin{figure}[!htp]
  \centering
  \includegraphics[width=\linewidth]{figure/img/varied-statistics.png} 
  \caption
    {
    1D Power Spectrum statistics from FaceForensics++ database.
    The statistical difference between two face manipulation algorithms sometimes are even larger than that between real and fake images.
    }
 \label{fig:varied-statics}
\end{figure}

==> table/tb_ff_attention.tex <==
\begin{figure}[t]
  \centering
    % \begin{minipage}{.21\textwidth}
        % \centering
        %  \includegraphics[width=0.5  \linewidth]{figure/pdf/att_example.pdf}
        %   \caption{The illustration of residual guided spatial attention maps.}
        %  \label{fig:att-example}
    % \end{minipage}%
    % \vspace{-5pt}
    % \hspace{0.5cm}
    % \begin{minipage}{0.68\textwidth}
    %   \centering
      \captionsetup{type=table}
      \caption{Comparison on FF++. The metric is AUC.}
      \scalebox{0.82}{
      \begin{tabular}{c|c|cccc} 
        \toprule
        \multirow{2}*{Training Set} & \multirow{2}*{Model} & \multicolumn{4}{c}{Testing Set} \\
        \cmidrule(lr){3-6}
        ~& ~& DF& F2F& FS& NT \\ 
        \midrule

        \multirow{3}*{DF}& 
        Xception~\cite{rossler2019faceforensics++}& \cellcolor{Gray}\textbf{0.993}& 0.736& 0.490& 0.736 \\
        % ~& Face X-ray~\cite{li2019face}& \cellcolor{Gray}0.987& 0.633& \textbf{0.600}& 0.698 \\
        ~& Face X-ray~\cite{li2019face}& \cellcolor{Gray}0.992&	\textbf{0.941}&	\textbf{0.753}&	\textbf{0.939}\\
        ~& Ours& \cellcolor{Gray}0.992& 0.764& 0.497& 0.814 \\
        \midrule

        \multirow{3}*{F2F}& Xception~\cite{rossler2019faceforensics++}& 0.803& \cellcolor{Gray}\textbf{0.994}& 0.762& 0.696 \\
        % ~& Face X-ray~\cite{li2019face}& 0.630& \cellcolor{Gray}0.984& 0.938& 0.945 \\
        ~& Face X-ray~\cite{li2019face}& \textbf{0.985}& \cellcolor{Gray}0.991& 0.727& 0.915 \\
        ~& Ours& 0.837& \cellcolor{Gray}\textbf{0.994}& \textbf{0.987}& \textbf{0.984} \\
        \midrule
	
        \multirow{3}*{FS}& 
        Xception~\cite{rossler2019faceforensics++}& 0.664& 0.888& \cellcolor{Gray}0.994& 0.713 \\
        % ~& Face X-ray~\cite{li2019face}& 0.458& 0.961& \cellcolor{Gray}0.981& 0.957 \\
        ~& Face X-ray~\cite{li2019face}& \textbf{0.938}& 0.923& \cellcolor{Gray}0.992& 0.866 \\
        ~& Ours& 0.685& \textbf{0.993}& \cellcolor{Gray}\textbf{0.995}& \textbf{0.980} \\
        \midrule

        \multirow{3}*{NT}& 
        Xception~\cite{rossler2019faceforensics++}& 0.799& 0.813& 0.731& \cellcolor{Gray}0.991 \\
        % ~& Face X-ray~\cite{li2019face}& 0.705& 0.917& 0.910& \cellcolor{Gray}0.925 \\
        ~& Face X-ray~\cite{li2019face}& \textbf{0.991}& 0.984& 0.706& \cellcolor{Gray}0.989 \\
        ~& Ours& 0.894& \textbf{0.995}& \textbf{0.993}& \cellcolor{Gray}\textbf{0.994} \\
        \bottomrule
      \end{tabular}}
      \label{tab:cmp-ff}
    % \end{minipage}
\end{figure}


==> table/tb_multi_task_high_frequency.tex <==
\begin{table}[tb!]
  \centering
    \begin{minipage}{0.45\textwidth}
      \centering
      \caption{Comparison on FF++ with methods using high-frequency features. The metric is accuracy.}
      \vspace{1mm}
      \scalebox{0.85}{
      \begin{tabular}{c|cccc} \toprule
        \multirow{2}*{Model} &\multicolumn{4}{c}{Testing Set (LQ)} \\
        \cmidrule(lr){2-5}
        ~& DF& F2F& FS& Real\\ 
        \midrule
        
        SRMNet~\cite{zhou2018learning} & 0.919& 0.927& 0.891& 0.693 \\
        Bayar Conv~\cite{10.1145/2909827.2930786} & 0.929& 0.946& 0.897& 0.755 \\
        SSTNet~\cite{wu2020sstnet} & 0.934& 0.919& 0.919& 0.793 \\
        % \midrule
         
        Ours & \textbf{0.986} &\textbf{0.957} & \textbf{0.929} & \textbf{0.971}\\
         \bottomrule
      \end{tabular}}
      \label{tab:cmp-residual}
    \end{minipage}
    \hspace{1cm}
    \begin{minipage}{.45\textwidth}
        \centering
      \caption{Comparison on FF++ with recent works using multi-task learning. The metric is accuracy.}
      \vspace{1mm}
      \scalebox{0.85}{
      \begin{tabular}{c|c|cc} \toprule
        \multirow{2}*{Training Set} & \multirow{2}*{Model} &\multicolumn{2}{c}{Testing Set} \\
        \cmidrule(lr){3-4}
        ~& ~& FS& F2F\\ 
        \midrule
        
        \multirow{5}*{F2F}& 
        LAE~\cite{du2019towards}& 0.632& \cellcolor{Gray}0.909 \\
        ~& ClassNSeg~\cite{nguyen2019multi} & 0.541& \cellcolor{Gray}0.928 \\
        ~& ForensicTrans~\cite{cozzolino2018forensictransfer} & 0.726& \cellcolor{Gray}0.945 \\
        % ~& MemoryNet~\cite{fernando2019exploiting} & 0.865& \cellcolor{Gray}0.987 \\
       % ~& Face X-ray~\cite{li2019face} & 0.857& \cellcolor{Gray}0.977 \\
        ~& Ours& \textbf{0.867} & \cellcolor{Gray}\textbf{0.992} \\
         \bottomrule
      \end{tabular}}
      \label{tab:cmp-generalization}
    \end{minipage}%
    
\end{table}

